LuxSQA: Ask Me in Luxembourgish with TTS-Augmented Spoken Question Answering

Spoken Question Answering (SQA) remains largely focused on high-resource languages and carefully recorded speech, limiting the reach of speech-LLM methods in low-resource settings. This paper investigates whether text-to-speech (TTS) can provide task-specific training data for Luxembourgish SQA without requiring a large human-recorded QA corpus. Starting from existing text-based QA resources, we translate questions into Luxembourgish, synthesize spoken questions with multiple TTS systems, and pair them with textual answers. We train a parameter-efficient SLAM-style architecture that connects a frozen Whisper encoder to frozen multilingual LLM backends through a learned projector and LoRA adapters. We compare MMS-TTS, Qwen3-TTS, and OmniVoice variants, including single-source corpora of about 48k questions and a 4TTS multi-source mix of approximately 230k questions. Evaluation on LLAMA-LB-Test with two real Luxembourgish speaker conditions shows that multi-source and voice-design-based synthetic training configurations yield the strongest SQA performance. The results also show that no-reference TTS quality scores do not monotonically predict downstream QA performance, indicating that synthetic speech must be evaluated as task-specific training data rather than only as natural-sounding audio.

==> plot.tex <==

\begin{figure*}[t]
\centering
\footnotesize
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=2 by 2,
        horizontal sep=1.2cm,
        vertical sep=1.1cm
    },
    width=0.47\textwidth,
    height=0.24\textwidth,
    ymin=0, ymax=100,
    ybar,
    bar width=4.2pt,
    enlarge x limits=0.06,
    xtick=data,
    ymajorgrids,
    grid style={gray!20},
    axis line style={black},
    tick align=outside,
    ylabel={Score (\%)},
    ylabel style={font=\bfseries\large},
    xlabel style={font=\bfseries\normalsize},
    title style={font=\bfseries\large},
    tick label style={font=\normalsize},
    xticklabel style={font=\footnotesize, rotate=45, anchor=east},
    legend style={
        font=\normalsize,
        draw=none,
        /tikz/every even column/.append style={column sep=0.8em}
    },
    legend columns=4,
    legend to name=qaLegend
]

% =========================
% Panel 1. Text baselines
% =========================
\nextgroupplot[
    title={Text baselines},
    symbolic x coords={A-noLB,E-noLB},
]
\addplot+[fill=blue!70] coordinates {
    (A-noLB,51.3)
    (E-noLB,51.6)
};
\addlegendentry{SemSim}

\addplot+[fill=orange!85] coordinates {
    (A-noLB,89.0)
    (E-noLB,83.5)
};
\addlegendentry{LLM Judge}

\addplot[black,dashed,thick] coordinates {
    (A-noLB,67.3) (E-noLB,67.3)
};
\addlegendentry{Base SemSim}

\addplot[black,dotted,thick] coordinates {
    (A-noLB,79.0) (E-noLB,79.0)
};
\addlegendentry{Base LLM Judge}

% =========================
% Panel 2. Generic LB-audio models
% =========================
\nextgroupplot[
    title={Generic LB-audio models},
    symbolic x coords={A-LB,E-LB},
]
\addplot+[fill=blue!70] coordinates {
    (A-LB,45.7)
    (E-LB,38.8)
};

\addplot+[fill=orange!85] coordinates {
    (A-LB,62.5)
    (E-LB,32.8)
};

\addplot[black,dashed,thick] coordinates {
    (A-LB,67.3) (E-LB,67.3)
};

\addplot[black,dotted,thick] coordinates {
    (A-LB,79.0) (E-LB,79.0)
};

% =========================
% Panel 3. Speaker 1
% =========================
\nextgroupplot[
    title={Speaker 1},
    symbolic x coords={
        E-4tts,
        E-qwenVD,
        A-4ttsASR,
        E-omniVD,
        E-scratch,
        E-omniCl,
        A-qwenVD,
        E-qwenCV,
        A-4tts,
        E-mtts,
        A-omniCl
    },
]
\addplot+[fill=blue!70] coordinates {
    (E-4tts,72.6)
    (E-qwenVD,72.0)
    (A-4ttsASR,71.7)
    (E-omniVD,70.7)
    (E-scratch,58.8)
    (E-omniCl,55.5)
    (A-qwenVD,51.9)
    (E-qwenCV,50.9)
    (A-4tts,50.8)
    (E-mtts,49.9)
    (A-omniCl,45.4)
};

\addplot+[fill=orange!85] coordinates {
    (E-4tts,60.1)
    (E-qwenVD,58.6)
    (A-4ttsASR,58.2)
    (E-omniVD,58.6)
    (E-scratch,35.3)
    (E-omniCl,32.7)
    (A-qwenVD,26.0)
    (E-qwenCV,25.4)
    (A-4tts,24.1)
    (E-mtts,24.3)
    (A-omniCl,18.6)
};

\addplot[black,dashed,thick] coordinates {
    (E-4tts,67.3) (A-omniCl,67.3)
};

\addplot[black,dotted,thick] coordinates {
    (E-4tts,79.0) (A-omniCl,79.0)
};

% =========================
% Panel 4. Speaker 2
% =========================
\nextgroupplot[
    title={Speaker 2},
    symbolic x coords={
        E-LoRA8ASR,
        E-4tts,
        E-qwenVD,
        A-4ttsASR,
        E-omniVD,
        E-scratch,
        A-qwenVD,
        E-omniCl,
        A-4tts,
        E-qwenCV,
        E-mtts,
        A-omniCl
    },
]
\addplot+[fill=blue!70] coordinates {
    (E-LoRA8ASR,74.8)
    (E-4tts,72.0)
    (E-qwenVD,71.7)
    (A-4ttsASR,70.9)
    (E-omniVD,67.8)
    (E-scratch,58.4)
    (A-qwenVD,51.8)
    (E-omniCl,51.3)
    (A-4tts,51.0)
    (E-qwenCV,48.5)
    (E-mtts,48.2)
    (A-omniCl,40.9)
};

\addplot+[fill=orange!85] coordinates {
    (E-LoRA8ASR,61.8)
    (E-4tts,60.2)
    (E-qwenVD,58.5)
    (A-4ttsASR,56.8)
    (E-omniVD,53.1)
    (E-scratch,35.4)
    (A-qwenVD,27.0)
    (E-omniCl,27.1)
    (A-4tts,24.0)
    (E-qwenCV,22.3)
    (E-mtts,21.6)
    (A-omniCl,16.3)
};

\addplot[black,dashed,thick] coordinates {
    (E-LoRA8ASR,67.3) (A-omniCl,67.3)
};

\addplot[black,dotted,thick] coordinates {
    (E-LoRA8ASR,79.0) (A-omniCl,79.0)
};

\end{groupplot}

\node[anchor=north] at ($(group c1r2.south)!0.5!(group c2r2.south)$)
{\pgfplotslegendfromname{qaLegend}};
\end{tikzpicture}

\caption{Compact QA evaluation bar plots on the LLAMA1-Test-Set. Each panel shows grouped vertical bars for Semantic Similarity and LLM Judge Mean. The dashed horizontal line marks the EuroLLM-9B base Semantic Similarity score, 67.3\%, and the dotted horizontal line marks the EuroLLM-9B base LLM Judge Mean, 79.0\%. Abbreviations: E = EuroLLM-9B, A = Apertus-8B, noLB = no \texttt{\_lb}, LB = \texttt{\_lb}, 4ttsASR = 4tts-from-asr, qwenVD = qwen-voicedesign, omniVD = omnivoice-voicedesign, omniCl = omnivoice-clone, qwenCV = qwen-customvoice, scratch = from-scratch.}
\label{fig:qa_barplots_compact}
\end{figure*}
